Identify As A Human Does: A Pathfinder of Next-Generation Anti-Cheat Framework for First-Person Shooter Games

The gaming industry has experienced substantial growth, but cheating in online games poses a significant threat to the integrity of the gaming experience. Cheating, particularly in first-person shooter (FPS) games, can lead to substantial losses for the game industry. Existing anti-cheat solutions have limitations, such as client-side hardware constraints, security risks, server-side unreliable methods, and both-sides suffer from a lack of comprehensive real-world datasets. To address these limitations, the paper proposes HAWK, a server-side FPS anti-cheat framework for the popular game CS:GO. HAWK utilizes machine learning techniques to mimic human experts' identification process, leverages novel multi-view features, and it is equipped with a well-defined workflow. The authors evaluate HAWK with the first large and real-world datasets containing multiple cheat types and cheating sophistication, and it exhibits promising efficiency and acceptable overheads, shorter ban times compared to the in-use anti-cheat, a significant reduction in manual labor, and the ability to capture cheaters who evaded official inspections.

==> Sections/Ethical_Consideration.tex <==
% \section{Ethics Considerations}\label{sec:ethical}
% The dataset only contains publicly accessible\footnote{\href{https://anonymized/}{Link}. We anonymize the platform’s URL and name.} information including in-game operations and data, and the banning information.
% %
% Its publication ensures no direct or indirect harm to the game, its distributors, players, or the community. The data provider has approved its release and reuse for research purposes, and no private information will be disclosed. 
% %
% %
% Still, we will anonymize all information to minimize the probability that may cause any unforeseen privacy concerns.
% %
% A data usage agreement will require users to commit to ethical, academic, and non-malicious use, with clear guidelines provided on ethical use and potential risks before using. 
% %
% The study adheres to local legislation and institutional requirements. 
% %
% % Written informed consent for participation was not required from the participants or the participants’ legal guardians/next of kin in accordance with the national legislation and institutional requirements.


% % \section{Compliance to Open Science Policy}\label{sec:openscience}
% % We open-source \sys and our datasets\footnote{\href{https://figshare.com/s/b41992b81a480337cab8}{Link}. The repository and dataset will be released upon acceptance. Artifacts are uploaded for the reference. Ethics statement is shown in \autoref{sec:ethical}.} to support open science.
% % %
% % We will make all links publicly available after paper acceptance.
% % %
% % Artifacts will be submitted to the Artifact Evaluation Committee for further review.

==> Sections/Keywords.tex <==
\begin{IEEEkeywords}
GameSecurity, Anti-Cheat, FPS games, feature extraction, time series prediction, classification
\end{IEEEkeywords}

==> Sections/References.tex <==
\bibliography{mybibliography}


==> Tables/RevStats_model_selection_Wallhack.tex <==
\begin{table*}[htbp]
\centering
\caption{Preliminary experimental result on the different model selection of \sysstats with the Wallhack dataset.} 
\label{tb:statswallhack}
\resizebox{\textwidth}{!}{%
\begin{tabular}{lcccccccccccccccccccccccccc}
\toprule
\multirow{2}{*}{\textbf{Model}} & \multicolumn{8}{c}{\textbf{Validation}} & \multicolumn{9}{c}{\textbf{Test}} \\
\cmidrule{2-9} \cmidrule{11-18}
& TP & TN & FP & FN & Recall & NPV & Accuracy & AUC-ROC & & TP & TN & FP & FN & Recall & NPV & Accuracy & AUC-ROC \\ 
\midrule
LogisticRegression & 714 & 7,629 & 1,116 & 253 & 0.738 & 0.968 & 0.859 & 0.805 && 943 & 5,622 & 3,627 & 82 & 0.920 & 0.986 & 0.639 & 0.764
\\
Naive Bayes & 604 & 7,677 & 1,068 & 363 & 0.625 & 0.955 & 0.853 & 0.751 & & 891 & 6,103 & 3,146 & 134 & 0.869 & 0.979 & 0.681 & 0.765 \\ 
RandomForest & 967 & 8,745 & 0 & 0 & 1 & 1 & 1 & 1 & & 751 & 8,083 & 1,166 & 274 & 0.733 & 0.967 & 0.860 & 0.803 
\\
SVM & 548 & 8,323 & 422 & 419 & 0.567 & 0.952 & 0.913 & 0.759 & & 817 & 7,227 & 2,022 & 208 & 0.797 & 0.972 & 0.783 & 0.789 
\\ 
MLP & 472 & 8,489 & 256 & 495 & 0.488 & 0.945 & 0.923 & 0.729 & & 788 & 7,726 & 1,523 & 237 & 0.769 & 0.970 & 0.829 & 0.802 
\\ 
GaussianNB & 604 & 7,677 & 1,068 & 363 & 0.625 & 0.955 & 0.853 & 0.751 & & 891 & 6,103 & 3,146 & 134 & 0.869 & 0.979 & 0.681 & 0.765
\\ 
QDA & 493 & 8,276 & 469 & 474 & 0.510 & 0.946 & 0.903 & 0.728 & & 815 & 7,270 & 1,979 & 210 & 0.795 & 0.972 & 0.787 & 0.791 \\ 
\sysstats & 604 & 8,241 & 504 & 363 & 0.625 & 0.958 & 0.911 & 0.783 & & 855 & 6,988 & 2,261 & 170 & 0.834 & 0.976 & 0.763 & 0.795 \\
\bottomrule
\end{tabular}
}%
\end{table*}


==> Tables/preliminary_experiments_datasets.tex <==
\begin{table}
\centering
\caption{Older batch of \textit{Aimbot} dataset descriptions for the preliminary experiments for \syspov and \sysstats. The number of people in \sysstats's Training set is fewer due to the simulation of balanced sampling.}
\label{tb:preliminary_dataset}
\begin{threeparttable}
\resizebox{0.47\textwidth}{!}{%
\begin{tabular}{lcccccccccccccc}
\toprule
\multicolumn{1}{c}{\multirow{2}{*}{\textbf{System}}} & \multicolumn{4}{c}{\textbf{Train}}
&  & \multicolumn{4}{c}{\textbf{Validation}}                                                                                   &  & \multicolumn{4}{c}{\textbf{Test}}                                                                                         \\ \cmidrule{2-5} \cmidrule{7-10} \cmidrule{12-15} 
\multicolumn{1}{c}{}                                    & \text{\#M\tnote{1}} & \text{\#P\tnote{2}} & \text{\#N\tnote{3}} & \text{\#C\tnote{4}} &  & \text{\#M\tnote{1}} & \text{\#P\tnote{2}} & \text{\#N\tnote{3}} & \text{\#C\tnote{4}} &  & \text{\#M\tnote{1}} & \text{\#P\tnote{2}} & \text{\#N\tnote{3}} & \text{\#C\tnote{4}} \\ \midrule 
\syspov&2,310&21,890&19,735&2,155&  &215&2,100&1,906&194&  &862&8,401&7,588&813\\
\sysstats&4,578&8,412&4,206&4,206&  &803&6,662&6,108&554&  &3,212&26,647&24,335&2,312\\
\bottomrule 
\end{tabular}
}
\raggedright \footnotesize
\textsuperscript{1}\textbf{\text{\#M}}: Number of matches;
\textsuperscript{2}\textbf{\text{\#P}}: Number of players in total;
\textsuperscript{3}\textbf{\text{\#N}}: Number of normal (honest) players;
\textsuperscript{4}\textbf{\text{\#C}}: Number of cheaters.
\end{threeparttable}
\end{table}
